Adam-Smith at SemEval-2023 Task 4: Discovering Human Values in Arguments with Ensembles of Transformer-based Models

This paper presents the best-performing approach alias "Adam Smith" for the SemEval-2023 Task 4: "Identification of Human Values behind Arguments". The goal of the task was to create systems that automatically identify the values within textual arguments. We train transformer-based models until they reach their loss minimum or f1-score maximum. Ensembling the models by selecting one global decision threshold that maximizes the f1-score leads to the best-performing system in the competition. Ensembling based on stacking with logistic regressions shows the best performance on an additional dataset provided to evaluate the robustness ("Nahj al-Balagha"). Apart from outlining the submitted system, we demonstrate that the use of the large ensemble model is not necessary and that the system size can be significantly reduced.

==> formulas/recall_macro.tex <==
\begin{equation}
recall_{macro} = \frac{1}{|L|}*\sum_{i=0}^{|L|}[recall_i]
\end{equation}

\begin{equation}
precision_{macro} = \frac{1}{|L|}*\sum_{i=0}^{|L|}[recall_i]
\end{equation}

==> tables/argument.tex <==
\begin{table}
\centering\small%
\setlength{\tabcolsep}{2.5pt}%
\begin{tabular}{@{}ll@{\hspace{10pt}}c@{\hspace{5pt}}cccccccccccccccccccccc@{}}
\toprule
\multicolumn{2}{@{}l}{\bf Preprocessing} & \bf  {\bf F1 Validation}  \\
\midrule
\multicolumn{2}{@{}l}{\emph{Training Before Data Update}} \\

& HUM1-96 IBM-Deberta-Large   & .516 \\
& HUM1-92 Microsoft Deberta Large  & \bf{.523} \\

& HCV-452 IBM-Roberta-large   & \bf{.529} \\
& HCV-399-Roberta-large  & .519 \\
\addlinespace

\multicolumn{2}{@{}l}{\emph{Ablation: After Data Update}} \\

& HCV-452 IBM-Deberta-Large   & \bf{.580} \\
& HCV-399-Microsoft Deberta Large  & .579 \\

& IBM-Roberta-large   & \bf{.579} \\
& Roberta-large  & .575 \\

\addlinespace

\bottomrule
\end{tabular}
\end{table}

==> tables/pretraining.tex <==
\begin{table}
\centering\small%
\setlength{\tabcolsep}{2.5pt}%
\begin{tabular}{@{}ll@{\hspace{10pt}}c@{\hspace{5pt}}cccccccccccccccccccccc@{}}
\toprule
\multicolumn{2}{@{}l}{\bf Pretraining} & \bf  {\bf F1 Validation}  \\
\midrule
\multicolumn{2}{@{}l}{\emph{Training Before Data Update}} \\

& HUM1-96 IBM-Deberta-Large   & .516 \\
& HUM1-92 Microsoft Deberta Large  & \bf{.523} \\

& HCV-452 IBM-Roberta-large   & \bf{.529} \\
& HCV-399-Roberta-large  & .519 \\
\addlinespace

\multicolumn{2}{@{}l}{\emph{Ablation: After Data Update}} \\

& HCV-452 IBM-Deberta-Large   & \bf{.580} \\
& HCV-399-Microsoft Deberta Large  & .579 \\

& IBM-Roberta-large   & \bf{.579} \\
& Roberta-large  & .575 \\

\addlinespace

\bottomrule
\end{tabular}
\caption{Pretraining Deberta: Before and after the training data update. The runs are based on different hyperparameters so only the direct comparison between pretrained and not-pretrained should be considered here.}
\label{pretraining}
\end{table}

==> tables/table_results_small.tex <==
\begin{table}[t]
\centering\small%
\setlength{\tabcolsep}{2.5pt}%
\begin{tabular}{@{}ll@{\hspace{10pt}}c@{\hspace{5pt}}cccccccccccccccccccccc@{}}
\toprule
\multicolumn{2}{@{}l}{\bf Test set / Approach} & \bf All \\
\midrule
\multicolumn{2}{@{}l}{\emph{Main}} \\
& \textcolor{gray}{Best per category} & \textcolor{gray}{.59}  \\
& \textcolor{gray}{Best approach} & \textcolor{gray}{.56}  \\
& \textcolor{gray}{BERT} & \textcolor{gray}{.42} & \\
& \textcolor{gray}{1-Baseline} & \textcolor{gray}{.26} \\
& EN-225-Thres-Train  & .56  \\
& EN-225-Log-Reg  & .54  \\
& EN-219-Thres-LoD (1st) & .56  \\
& EN-233-Silver-Labels & .54 \\
\addlinespace
\multicolumn{2}{@{}l}{\emph{Nahj al-Balagha}} \\
& \textcolor{gray}{Best per category} & \textcolor{gray}{.48}  \\
& \textcolor{gray}{Best approach} & \textcolor{gray}{.40}  \\
& \textcolor{gray}{BERT} & \textcolor{gray}{.28}  \\
& \textcolor{gray}{1-Baseline} & \textcolor{gray}{.13}  \\
& EN-225 T-Train & .36  \\
& EN-225-Log-Reg (1st) & .40  \\
& EN-219-Thres-LoD & .34  \\
& EN-233 & .34  \\
\addlinespace
\multicolumn{2}{@{}l}{\emph{New York Times}} \\
& \textcolor{gray}{Best per category} & \textcolor{gray}{.47} \\
& \textcolor{gray}{Best approach} & \textcolor{gray}{.34} \\
& \textcolor{gray}{BERT} & \textcolor{gray}{.24} \\
& \textcolor{gray}{1-Baseline} & \textcolor{gray}{.15} \\
&  EN-225 T-Train & .26 \\
& EN-225-Log-Reg & .27 \\
& EN-219-Thres-LoD & .25  \\
& EN-233 & .24  \\
\bottomrule
\end{tabular}
\caption{Achieved F$_1$-score of team adam-smith per test dataset. Approaches marked with * were not part of the official evaluation. Approaches in gray are shown for comparison: an ensemble using the best participant approach for each individual category; the best participant approach; and the organizer's BERT and 1-Baseline.}
\label{table-results-small}
\end{table}

